Projectron -- A Shallow and Interpretable Network for Classifying Medical Images

This paper introduces the `Projectron' as a new neural network architecture that uses Radon projections to both classify and represent medical images. The motivation is to build shallow networks which are more interpretable in the medical imaging domain. Radon transform is an established technique that can reconstruct images from parallel projections. The Projectron first applies global Radon transform to each image using equidistant angles and then feeds these transformations for encoding to a single layer of neurons followed by a layer of suitable kernels to facilitate a linear separation of projections. Finally, the Projectron provides the output of the encoding as an input to two more layers for final classification. We validate the Projectron on five publicly available datasets, a general dataset (namely MNIST) and four medical datasets (namely Emphysema, IDC, IRMA, and Pneumonia). The results are encouraging as we compared the Projectron's performance against MLPs with raw images and Radon projections as inputs, respectively. Experiments clearly demonstrate the potential of the proposed Projectron for representing/classifying medical images.

==> old_results1.tex <==
\begin{table}[h]
\normalsize
\caption{Results for Projectron against other published techniques (sorted in ascending order of \textit{Accuracy}).}
\begin{tabular}{lc}
\hline
\hline
\multicolumn{2}{c}{\textbf{MNIST Dataset}}                                    \\ \hline
\multicolumn{2}{c}{(60,000 images training and 10,000 images for testing)}    \\ \hline
Method                           & Accuracy               \\ \hline
Projectron                       & $94.75\%$                       \\
MLP+Raw                        & $97.89\%$                       \\ 
MLP+Radon                    & $96.81\%$                       \\ \hline
%DropConnect \cite{wan2013regularization} & $99.79\%$      \\ \hline
\multicolumn{2}{c}{\textbf{CT Emphysema Dataset}}         \\ \hline
\multicolumn{2}{c}{(168 images for training/testing)}     \\ \hline
Method                           & $A_{CT}$               \\ \hline
Projectron                       & $59.00\%$                       \\
MLP+Raw                              &  $57.73\%$                      \\ 
MLP+Radon                    & $60.12\%$                       \\ \hline
%VGG16-FCL                        & 69.64\%                \\ \hline
\multicolumn{2}{c}{\textbf{Invasive Ductal Carcinoma}}                        \\ \hline
\multicolumn{2}{c}{(114,235 images for training and 50,963 images for testing)} \\ \hline
Method                           & Accuracy               \\ \hline
Projectron                       & $78.00\%$                       \\
MLP+Raw                              & $71.35\%$                       \\ 
MLP+Radon                    & $71.35\%$                       \\ \hline
%CNN \cite{cruz2014automatic}     & $84.23\%$              \\ \hline
\multicolumn{2}{c}{\textbf{IRMA Dataset}}                                     \\ \hline
\multicolumn{2}{c}{(12,677 images for training and 1,733 images for testing)} \\ \hline
Method                           & $A_{IRMA}$             \\ \hline
Projectron                       & $69.00\%$                       \\
MLP+Raw                            & $41.23\%$                       \\
MLP+Radon                    & $47.02\%$                       \\ \hline
%VGG16-FC7                        & 84.58\%                \\ 
%CNN + Radon                      & 90.30\%                \\ \hline
\multicolumn{2}{c}{\textbf{Pneumonia Dataset}}                                \\ \hline
\multicolumn{2}{c}{(5,216 images for training and 624 images for testing)}    \\ \hline
Method                           & Accuracy               \\ \hline
Projectron                       & $70.03\%$                       \\
MLP+Raw                              &  $37.50\%$                      \\
MLP+Radon                    & $37.50\%$                       \\ \hline
%CNN                              &                        \\ \hline
%\multicolumn{2}{c}{\textbf{BreakHis Dataset}}                                 \\ \hline
%\multicolumn{2}{c}{(Train and test distribution across five folds)} \\ \hline
%Method                           & Averaged Accuracy               \\ \hline
%Projectron                       &                        \\
%MLP+Raw                              &                        \\
%MLP+Radon                              &                        \\ 
\hline
\hline
\end{tabular}
\label{tab:final_results}
\end{table}

==> old_results2.tex <==
\begin{table}[h]
\normalsize
\caption{Results for Projectron against other published techniques (sorted in ascending order of \textit{Accuracy}).}
\begin{tabular}{llll}
\hline
\hline
\multicolumn{4}{c}{\textbf{MNIST Dataset}}                                                                     \\ \hline
\multicolumn{4}{c}{(60,000 images training and 10,000 images for testing)}                                     \\ \hline
Method                     & Accuracy                     & $\lvert h \rvert$                     & Training Time                     \\ \hline
Projectron                 & 94.75\%                      & 1,196,100                       & 141.96s                          \\
MLP+Raw                    & 97.89\%                      & 311,650                        & 4min 18s                         \\
MLP+Radon                  & 96.81\%                      & 117,850                         & 1min 39s                         \\ \hline
\multicolumn{4}{c}{\textbf{CT Emphysema Dataset}}                                                              \\ \hline
\multicolumn{4}{c}{(168 images for training/testing)}                                                          \\ \hline
Method                     & Accuracy                     & $\lvert h \rvert$                     & Training Time                     \\ \hline
Projectron                 & $59.00\%$                             &                         &                          \\
MLP+Raw                    & $57.73\%$                             &                         &                          \\
MLP+Radon                  & $60.12\%$                             &                         &                          \\ \hline
\multicolumn{4}{c}{\textbf{Invasive Ductal Carcinoma}}                                                         \\ \hline
\multicolumn{4}{l}{(114,235 images for training and 50,963 images for testing)}                                \\ \hline
Method                     & Accuracy                     & $\lvert h \rvert$                     & Training Time                     \\ \hline
Projectron                 &  $78.00\%$                            &                         &                          \\
MLP+Raw                    & $71.35\%$                             & 3,128,752                        & 50min 54s                         \\
MLP+Radon                  & $71.35\%$                             & 364,232                        & 11min 19s                         \\ \hline
\multicolumn{4}{c}{\textbf{IRMA Dataset}}                                                                      \\ \hline
\multicolumn{4}{l}{(12,677 images for training and 1,733 images for testing)}                                  \\ \hline
Method                     & Accuracy                     & $\lvert h \rvert$                     & Training Time                     \\ \hline
Projectron                 & $69.00\%$                             &                         &                          \\
MLP+Raw                    & $41.23\%$                             &                         &                          \\
MLP+Radon                  & $47.02\%$                             & 3,187,449                        & 10min 34s                         \\ \hline
\multicolumn{4}{c}{\textbf{Pneumonia Dataset}}                                                                 \\ \hline
\multicolumn{4}{l}{(5,216 images for training and 624 images for testing)}                                     \\ \hline
Method                     & Accuracy                     & $\lvert h \rvert$                     & Training Time                     \\ \hline
Projectron                 & $70.03\%$                             &                         &                          \\
MLP+Raw                    & $37.50\%$                             & 253,158,752                         &                          \\
MLP+Radon                  & $37.50\%$                              & 3,270,404                         & 4min 32s                         \\ 
\hline
\hline
\end{tabular}
\label{tab:final_results}
\end{table}
